Checking Phylogenetic Decisiveness in Theory and in Practice

Suppose we have a set $X$ consisting of $n$ taxa and we are given information from $k$ loci from which to construct a phylogeny for $X$. Each locus offers information for only a fraction of the taxa. The question is whether this data suffices to construct a reliable phylogeny. The decisiveness problem expresses this question combinatorially. Although a precise characterization of decisiveness is known, the complexity of the problem is open. Here we relate decisiveness to a hypergraph coloring problem. We use this idea to (1) obtain lower bounds on the amount of coverage needed to achieve decisiveness, (2) devise an exact algorithm for decisiveness, (3) develop problem reduction rules, and use them to obtain efficient algorithms for inputs with few loci, and (4) devise an integer linear programming formulation of the decisiveness problem, which allows us to analyze data sets that arise in practice.

==> Sections/algorithms.tex <==
% !TEX root = ../isbra20MainBFBP.tex

\section{An Exact Exponential Algorithm to Solve Rainbow Coloring}

Assume we want to color $n$ vertices in a 3-uniform hypergraph, using 3 different colors. By the pigeonhole principle, there exists a color that is used at most $n/3$ times. In this Algorithm, we try all colorings in which color 1 is used up to $n/3$ times and we assume we are not using color 1 anymore, after that we manage the other 2 colors to see if there exists a non-rainbow coloring for the given graph or not.

After using the first color for $i$ time ($1\leq i \leq n/3$) there will be 4 different groups of hyperedges based on the number of colored vertices:  The hyperegdes with zero, one, two or all three colored vertices.

The only group that may cause a rainbow color is group 2, so if there is no hyperedge in group 2, we can color the rest of the vertices arbitrarily and the result is a non-rainbow coloring for the graph. But if there is at least one hyperedge in group 2, we know the other two vertices in that must have the same color, so we take one hyperedge in group 2 and color the two uncolored hyperedges by color 2. Doing this may result in having hyperedges with exactly one vertex in color 1, exactly one vertex in color 2 and exactly one uncolored vertex. Now we need to find all these hyperedges and color the third hyperedge by color 2 since coloring them by color 3 will result in a rainbow. We continue until we have no hyperedge with the mentioned property. At this point, if there is no more uncolored vertices, it means we failed using three colors to have a non-rainbow coloring and there is no non-rainbow coloring for the given hypergraph, and if there still exist some uncolored vertices, we color all them using color 3 and the result is a non-rainbow coloring. The following is the pseudocode of the given algorithm:

\begin{algorithm}%[H]
\SetAlgoLined
\SetNoFillComment
\DontPrintSemicolon


\For {$i = 1$  \KwTo $\frac{n}{3}$}{
\ForEach {subset of size $i$ of set $V$}
{ Use color 1 to color all the vertices in the chosen subset\\
\If {there is no hyperedge with exactly one vertex with color}
{ randomly distribute color 2 and 3 among uncolored vertices\\
\Return $H$
}
}
\Else{
Pick one hyperedge with one colored vertex and use color 2 for the other two vertices\\
\While{There exists a hyperedge with one color 1 , one color 2 and an uncolored vertex}{
Pick a hyperedge with one color 1, one color 2 and one uncolored vertex and use color 2 for coloring the third vertex\\
}
\If{there are no uncolored vertices}{
\Return "there does not exist any no-rainbow coloring for $H$"\\
}
\Else{
Color all the remaining vertices with color 3\\
\Return $H$
}
}
}
\caption{\texttt{Non-rainbow Coloring of}$(H)$ with 3 colors}
\end{algorithm}

The two \textbf{for} loops dominate the running time of this algorithm. For any $i$ from 1 to $\frac{n}{3}$ we choose any $i$ nodes from $n$ nodes which means we have $\sum_{i=1}^{n/3} {n \choose i}$ repeats which gives $O(1.7^n)$.

Now we generalize the algorithm for the case of $r=4$ which means each hyperedge contains 4 vertices and we have 4 different colors to color the vertices. By the Pigeonhole Principle, we know there is a color that is used at
most $\frac{n}{4}$ times. So at first we color any choice of $i$ vertices with color 1, when $i$ can vary from $1$ to $\frac{n}{4}$. After this step, there are $n-i$ uncolored vertices and we know there exists another color that is used at most $\frac{n-i}{3}$ times, so we color any choice of $j$ vertices with color 2, when $j$ can vary from 1 to $\frac{n-i}{3}$. Now we are done with the first 2 colors and we are allowed to only use color 3 and 4 for coloring the rest of vertices. 
But what hyperedges have the chance of making a rainbow? The only group of hyperedges in which rainbow may occur are the ones with exactly one vertex in color 1, exactly one vertex in color 2 and exactly 2 uncolored vertices.
If there is no such a hyperedge we can easily distribute color 3 and 4 on the remaining vertices and the result will be a non-rainbow coloring, but when we have hyperedges with this property we need to apply an algorithm to avoid non-rainbow coloring.
First we find one hyperedge with this property and color the 2 uncolored vertices by color 3. After that we try to find the hyperedges with 3 colored vertices, one by color 1, one by color 2 and the third by color 3. 
Since we are not allowed to use color 1 and 2 anymore and coloring the fourth vertex using color 4 will make a rainbow hyperedge, we color the last vertex in the hyperedge by color 3 as well. We continue doing that until no
other uncolored vertices remain or if no other hyperedge with exactly three colored vertices (each vertex by a different color), exists. If there are no more vertices, we have failed using color 4 and there is no non-rainbow coloring for this hypergraph. If there are some uncolored vertices but there is no hyperedge with exactly one color 1, exactly one color 2, exactly one color 3 and one uncolored vertex, we can use color 4 for the rest of the vertices and the result will be a no-rainbow coloring for the graph. Algorithm \ref{alg:nonRainbow} shows the relevant pseudocode.



\begin{algorithm}%[H]
\SetAlgoLined
\SetNoFillComment
\DontPrintSemicolon


\For {$i = 1$  \KwTo $\frac{n}{4}$}{
\ForEach {subset of size $i$ of set $V$}
{ Use color 1 to color all the vertices in the chosen subset\\

\For {$j = 1$ \KwTo $\frac{n-i}{3}$}{
\ForEach {subset of size $j$ of set $V$}
{Use color 2 to color all the vertices in the chosen subset\\


\If {there is no hyperedge with exactly one vertex with color 1 and exactly one vertex with color 2}
{ randomly distribute color 3 and 4 among uncolored vertices\\
\Return $H$
}
\Else{
Pick one hyperedge with one colored vertex with color 1 and one colored vertex with color 2 and use color 3 for the other two vertices\\
\While{there exists a hyperedge with one color 1, one color 2, one color 3 and an uncolored vertex}{
Pick a hyperedge with one color 1, one color 2, one color 3 and one uncolored vertex and use color 3 for coloring the fourth vertex\\
}
\If{There does not exist any uncolored vertices}{
\Return ``there does not exist any no-rainbow coloring for $H$"\\
}
\Else{
Color all the remaining vertices with color 4\\
\Return $H$
}
}
}
}

}
}
\caption{\texttt{Non-rainbow Coloring of}$(H)$ with 4 colors.\label{alg:nonRainbow}}
\end{algorithm}

In the given algorithm, three for loops, determine the running time of this algorithm. For any $i$ from 1 to $\frac{n}{3}$ we choose any $i$ nodes from $n$ nodes and then for any $j$ from 1 to $\frac{n-i}{3}$ we choose any $j$ vertices which means we have $\sum_{i=1}^{n/3} {n \choose i} \sum_{j=1}^{n-i/4} {n-i \choose j}$ repeats which gives $O()$.





==> Sections/preamble.tex <==
\usepackage{amssymb,amsmath,amsfonts}
%\usepackage{amsthm}
%\usepackage{newtxtext,newtxmath}
\usepackage{latexsym}
\usepackage{verbatim}
\usepackage{enumerate}
\usepackage{url}
\usepackage[ruled,linesnumbered,noend]{algorithm2e}
\usepackage{color}


\newcommand{\COLOR}{\ensuremath{{\rm color}}}
\newcommand{\COUNT}{\ensuremath{{\rm count}}}

\newcommand{\ROOT}{\ensuremath{{\rm root}}}
\newcommand{\Cl}{\ensuremath{{\mathrm{Cl}}}} 		% Clusters
\newcommand{\true}{{\ensuremath{\texttt{true}}}}
\newcommand{\false}{\ensuremath{\texttt{false}}}
\newcommand{\NULL}{\ensuremath{\texttt{null}}}
\newcommand{\MP}{\ensuremath{M_\P}} % Size of a profile
\newcommand{\TG}{\ensuremath{\Gamma}} % Triple graph 
\newcommand{\cd}{\ensuremath{{\mathrm{cd}}}} % Coverage density
\newcommand{\Spl}{\ensuremath{{\mathrm{Spl}}}} % Split set

\renewcommand{\P}{\ensuremath{\mathcal{P}}} 
\newcommand{\DG}{\ensuremath{H_\P}} % Display Graph

\renewcommand{\S}{\ensuremath{\mathcal{S}}} 


\newtheorem{observation}{Observation}
%\theoremstyle{remark}
\newtheorem{rem}{Remark}
\theoremstyle{definition}
\newtheorem{definition}{Definition}
\newtheorem{example}{Example}


==> Sections/sat.tex <==
% !TEX root = ../isbra20MainBFBP.tex
\section{Using Satisfiability\label{sec:satisfiability}}

The na\"ive way to use Theorem \ref{thm:decisiveness} to test whether a coverage pattern $\S$ is decisive is to enumerate all partitions of $X$ into four non-empty sets $A_1, A_2, A_3, A_4$ and verify that there is a set $Y \in \S$ that intersects each $A_i$.  Equivalently, by Proposition \ref{lem:decRain}, we can enumerate all surjective colorings of $H(S)$ and check if each of these colorings yields a rainbow edge.  In either approach, the number of options to consider is given by a Stirling number of the second kind, namely $\left\{{n \atop 4}\right\} \sim \frac{4^n}{4!}$ \cite{GrahamKnuthPatashnik1989}.  Here we show how a substantial improvement on exhaustive enumeration is possible.

\begin{theorem}\label{thm:decSat}
Let $\S$ be a taxon coverage pattern for a taxon set $X$.  Then, there is an algorithm that, in $O(1.78^n)$ time determines whether or not $\S$ is decisive, where $n = |X|$.
\end{theorem}

The proof of Theorem \ref{thm:decSat} uses a reduction from decisiveness to
$k$-SAT, the well-known problem of determining whether a Boolean formula in conjunctive normal form (CNF) with at most $k$ variables per clause is satisfiable. $k$-SAT is, of course, NP-complete for $k \ge 3$ --- and, thus, unlikely to have a polynomial-time algorithm.  On the other hand, however, there algorithms for $k$-SAT that vastly improve on trivial enumeration \cite{SchoeningToran2013}.  Here, for concreteness, we use the fact that $k$-SAT on an $n$-variable formula can be solved in $O^*\left ( \left (\frac{2k}{k+1}\right)^n \right)$ time\footnote{The $O^*$-notation is a variant of $O$-notation that ignores polynomial factors \cite{FominKratsch2010}.} deterministically and in $O^*\left ( \left (\frac{2(k-1)}{k}\right)^n \right)$ time probabilistically \cite{SchoeningToran2013}. %Note, however, that asymptotically faster algorithms exist \FIX{REFS?}.

We exploit the connection between decisiveness and the $4$-NRC problem given in Proposition \ref{lem:decRain}.  In addition to $4$-NRC, we also consider $3$-NRC, since that case will be useful later.
To simplify the exposition, we only consider 3-NRC and 4-NRC for 3-uniform and 4-uniform hypergraphs, respectively; however, note that the same asymptotic time bounds carry over to the non-uniform case. 

\begin{lemma}\label{lem:ColorSat}
3-NRC is reducible to 5-SAT and 4-NRC is reducible to 8-SAT.
\end{lemma}

\begin{proof}
%Let $H = (X,E)$ be the input hypergraph.  For $r=3$, we first verify that $|E| \geq {n-1 \choose 2}$; if not, the bound given in Section \ref{sec:bound}, implies that the hypergraph is 3-nrc. If $|E| \geq {n-1 \choose 2}$, we represent the color of each vertex $v_i$ by a 2-digit binary string $c(v_i) = x_iy_i$ where $x_i$, $y_i \in \{0,1\}$. We represent each of our three colors with a 2-digit binary string, coding colors 1, 2, and 3 as 00, 01, and 10, respectively.  Consider any hyperedge $e = \{v_1, v_2,v_3\}$. To ensure that at least two of $e$'s nodes share a color, we add the following constraints:
%%That is, if $e = \{v_1, v_2,v_3\}$, we must have either  $c(v_1) = c(v_2)$ or $c(v_1) = c(v_3)$ or $c(v_2) = c(v_3)$. 
%%Now if we use the binary representation of each vertices' color we have: 
%$((x_1 = x_2 ) \wedge (y_1 = y_2)) \vee ((x_1 = x_3) \wedge (y_1 = y_3)) \vee ( (x_2= x_3) \wedge (y_2 = y_3)) $.
%We can transform the resulting expression to a 5-CNF formula (see Appendix).  We then obtain a formula for the entire hypergraph by taking the conjunction of the expressions for all the hyperedges. Note, however, that this formula is trivially satisfied by assigning the same color to all nodes.  To ensure that each color is used at least once, we arbitrary pick a node $v \in X$ and assign it color 1.  We then consider every pair of nodes $u, w \in X \setminus \{v\}$ and assign one of them color 2 and the other color 3.  For each such pair, we have a 5-CNF formula, where some of  the variables become fixed.  Solving 5-SAT takes $O^*((\frac{10}{6})^n) = O(1.67^n)$ time. Since only $O(n^2)$ pairs $u,w$ are considered, the total time to solve these formulas is $O^*(1.67^n)$. If any of the formulas is satisfiable, then the hypergraph has a no-rainbow coloring.
%
We only show the  reduction for 4-NRC.  The reduction for 3-NRC is analogous.  

If $|E| < {n-1 \choose 3}$, Lemma \ref{thm:lowerBound}, of Section \ref{sec:bound}, implies that $H$ admits a 4-no-rainbow coloring, and we are done. Otherwise, we encode the color of each vertex $v_i$ by a 2-digit binary string $c(v_i) = x_iy_i$ where $x_i$, $y_i \in \{0,1\}$, and we represent each of our four colors with a 2-digit binary string, coding colors 1, 2, and 3 as 00, 01, 10, and 11, respectively.   For each hyperedge $e = \{v_1, v_2, v_3, v_4\}$ we must have  $c(v_1) = c(v_2)$ or $c(v_1) = c(v_3)$ or  $c(v_1) = c(v_4)$ or $c(v_2) = c(v_3)$ or $c(v_2) = c(v_4)$ or $c(v_3) = c(v_4)$, which is expressed as:
 $$((x_1 = x_2 ) \wedge (y_1 = y_2)) \vee ((x_1 = x_3) \wedge (y_1 = y_3)) \vee  ((x_1 = x_4) \wedge (y_1 = y_4))$$
 $$ \vee ( (x_2= x_3) \wedge (y_2 = y_3)) \vee ((x_2 = x_4) \wedge (y_2 = y_4)) \vee ((x_3 = x_4) \wedge (y_3 = y_4)) .$$
It is straightforward to transform the above formula to an 8-CNF formula (see the Appendix). We then obtain a formula for the entire hypergraph by taking the conjunction of the expressions for all the hyperedges. 
Note, however, that the resulting formula is trivially satisfied by assigning the same color to all nodes.  To ensure that each color is used at least once, we arbitrary pick a node $v \in X$ and assign it color 1.  We then consider every triple of nodes $u, w, x \in X \setminus \{v\}$ and assign them colors 2, 3, and 4, respectively.  For each such pair, we have a 8-CNF formula, where some of  the variables become fixed.  Solving 8-SAT takes time $O^*((\frac{16}{9})^n) = O(1.78^n)$.
\QED 
\end{proof}
 
\begin{proof}[of Theorem \ref{thm:decSat}]
Follows from Lemma \ref{lem:ColorSat} and Proposition \ref{lem:decRain}. 
\QED 
\end{proof}
 
We note that, the formulation of decisiveness as a satisfiability problem described in proving Theorem \ref{thm:decSat} offers another potentially useful option in practice: it enables us to benefit from satisfiability solver technology, which has achieved considerable sophistication \cite{GomesEtAlSatisfiability2008,MalikZhang_Satisfiability2009}.



==> Sections/someresults.tex <==
% !TEX root = ../isbra20MainBFBP.tex
\section{Some Results}

It is convenient to consider hypergraph colorings that are defined for only a subset of the nodes.  A \emph{partial $r$-coloring} of a hypergraph $H = (X,E)$ is a mapping $c$ from a subset of $X$ to $[r]$.
A node $v \in X$ is \emph{colored} if $c(v)$ is defined. An edge $e \in E$ is \emph{fully-colored} if $c(v)$ is defined for each $v \in e$.  Edge $e$ is \emph{almost colored} if $c(v)$ is undefined for exactly one node $v \in e$.

A \emph{valid initial coloring} of $H = (X,E)$ is a partial coloring $c$ such that (i) for each $i \in [r]$ there is precisely one node $v_i \in X$ such that $c(v_i) = i$ and (ii) no fully-colored edge $e \in E$ is rainbow colored.   

\begin{observation}
If hypergraph $H$ has no valid initial coloring, then $H$  does not admit a no-rainbow $r$-coloring.
\end{observation}

\begin{lemma}
Let $c$ be a partial coloring of $H$.  For each $i \in [r]$ and $r\leq 3$, let $F_i = \{e \in E: c(v) = i, \text{ for some } v \in e\}$. Assume that for each $i \in [r]$ there exists at least one $v \in V$ such that $c(v) =i$.  Suppose that $F_i \cap F_j = \emptyset$  for any $i, j \in [r]$, $i \neq j$.  Then, $H$ has a no-rainbow $r$-coloring.
\end{lemma}

\begin{proof}
For each $v \in V$ such that $c(v)$ is undefined, make $c(v) = k$ such that $k \neq i$ and $k \neq j$.  Thus, every vertex is now colored.  We need to verify that there is no rainbow colored edge.
\end{proof}


\begin{lemma}  Let $H=(X,E)$ be an $r$-regular hypergraph such that, for each $i \in [r]$, there is exactly one node such that $c(v) = i$, and there is no edge $e \in E$ such that $c(x) = c(y)$ for any two distinct colored nodes $x, y \in e$. 
Suppose that every almost-colored edge $e \in E$ contains two colored nodes $u, v$ such that $c(u) = c(v)$. Then, $H$ has a non-rainbow $r$-coloring.
\end{lemma}

\begin{proof}
@@@
\end{proof}
